Clinical Document Classification Using Labeled and Unlabeled Data Across Hospitals

Reviewing radiology reports in emergency departments is an essential but laborious task. Timely follow-up of patients with abnormal cases in their radiology reports may dramatically affect the patient's outcome, especially if they have been discharged with a different initial diagnosis. Machine learning approaches have been devised to expedite the process and detect the cases that demand instant follow up. However, these approaches require a large amount of labeled data to train reliable predictive models. Preparing such a large dataset, which needs to be manually annotated by health professionals, is costly and time-consuming. This paper investigates a semi-supervised learning framework for radiology report classification across three hospitals. The main goal is to leverage clinical unlabeled data in order to augment the learning process where limited labeled data is available. To further improve the classification performance, we also integrate a transfer learning technique into the semi-supervised learning pipeline . Our experimental findings show that (1) convolutional neural networks (CNNs), while being independent of any problem-specific feature engineering, achieve significantly higher effectiveness compared to conventional supervised learning approaches, (2) leveraging unlabeled data in training a CNN-based classifier reduces the dependency on labeled data by more than 50% to reach the same performance of a fully supervised CNN, and (3) transferring the knowledge gained from available labeled data in an external source hospital significantly improves the performance of a semi-supervised CNN model over their fully supervised counterparts in a target hospital.

==> discussion.tex <==
% !TEX root = main_ssltran.tex
%\section*{Discussion}
\label{sect:discussion}

%\hl{shows examples of radiology reports in which supervised ML models failed to detect abnormality.}


%The results of our empirical investigation highlight the key role of the combined semi-supervised transfer learning approach not only in dealing with the scarcity of labeled data, but also in significantly increasing the classification performance. 
%The misclassfied examples, shown in \hl{Figure (Table?) XX}, demonstrate that the conventional supervised approaches have faced key challenges in detecting abnormalities from radiology reports. 
%We found that leveraging unlabeled data from the target domain along with the available labeled data from other resources, can significantly improve the abnormality detection task. 
%Our results suggest that such approach also reduces the amount of labeled data required for training an initial learning model, which can further translates into less manual annotation effort.  



%- discuss the difference between hospitals data


%- say sth about GCH: no labeled data??


%- discuss how random selection in ssl reduce the need  of labeled data

%In order to better understand the difference in the performances of the supervised approaches for abnormality detection task, we performed a paired t-test over the best and the second-best performing models on each dataset (i.e., between CNN and SGD over RBWH and between CNN and SVM over RCH). The results showed that CNN performed significantly better than the rest of the classifiers (i.e., $p$-$value=0.044 < 0.05$) on RBWH data. However, this conclusion cannot be drawn on RCH data (i.e., $p$-$value=0.291 > 0.05$).

%Comparing the results in Table~\ref{tab:supres} and Table~\ref{tab:sslres} revealed that both SSL approaches surpassed the best supervised model with approx. 1\% to 2\% improvement on F1-Score on both datasets, but not statistically significant (i.e., $p$-$values> 0.05$). Furthermore, the difference between the two proposed SSL approaches were not significant.

%In the course of the experiments it became apparent that the learning models can be biased towards predicting one class more than the other for the instances in the unlabelled set. In addition, it is more probable to have normal cases than abnormal cases in the collected data from EDs (e.g., Table~\ref{tab:regresnewdata} showed that the distribution of the normal cases in the labelled sets of RBWH and RCH are 58\% and 66\%, respectively). Since detecting the less distributed abnormal cases is the dominant task of the model, further investigation to understand the effect of a more balanced selection scenario in the proposed SSL framework would be warranted. In order to select the same portion of the normal and abnormal cases from the unlabelled set during the SSL procedure, the least predicted classes by a model was identified. Before retraining the model over the newly populated labelled data, a balancing component was added to under-sample the most frequently predicted class to the number of the least predicted class. This ensures that the same number of instances from normal and abnormal cases are selected and passed to train the model in every SSL loop. The results showed that balanced selection of the instances relatively improved (but not significantly) the performance of the SSL approaches (except ensemble-based SSL on RCH). On RBWH dataset, the balanced self-trained SSL and the balanced ensemble-based SSL achieved 0.9177 and  0.9166 F1-Scores, respectively, and on RCH, the balanced self-trained SSL achieved 0.9486 F1-Score, which are in general approx. 0.002 improvement over the unbalanced versions of SSL.

%A comparison to the state-of-the-art approach on the same dataset~\cite{koopman2015automated} showed that the proposed SSL approaches surpassed their approach with 0.03 improvement in F1-Score on RBWH dataset while on RCH achieved on par results (i.e., 0.95 F1-Score). Their classifier was a finely tuned SVM that employs sophisticated engineered features for the task (i.e., from syntactic features to semantic features using external resources such as SNOMED CT ontology).

%\begin{table*}
%\small
%\centering
%\caption{Balanced semi-supervised approaches performance}%-  (full gird)
%\label{tab:sslres}
%\begin{tabular}{lllllll}
%\toprule
%\multirow{2}{*}{} & \multicolumn{3}{c}{RBWH}          & \multicolumn{3}{c}{RCH}           \\ 
%                  & P      & R      & F1              & P      & R      & F1              \\ \hline
%Balanced Sef-trained SSL               & 0.9321 & \textbf{0.9045}  & \textbf{0.9177}   & \textbf{0.9465} & 0.9526 & 0.9486 \\ \hline
%Balanced Ensemble-based SSL               & \textbf{0.925} & 0.9094 & 0.9166 & 0.9491 & \textbf{0.9588}  & \textbf{0.9523}  \\
%\bottomrule
%\end{tabular}
%\end{table*}

%The results have shown that incorporating unlabelled samples through a semi-supervised framework can lead to classifiers with higher performance compared to when only using labelled samples to train classification models.

%?	Balancing
%?	Across-hospital evaluation




% \begin{table}[]
% \small
% \centering
% \caption{Transfer Semi-supervised Learning on RBWH as target hospital } %(full grid)
% \label{tab:tlwithft}
% \begin{tabular}{cl|llll}
% \multicolumn{2}{l|}{\multirow{2}{*}{}} & \multicolumn{4}{c}{Unlabelled} \\
% \multicolumn{2}{l|}{}                  & RBWH\_U   & RCH\_U  & AudeGen & ALL \\
% \midrule
% \multirow{2}{*}{\rotatebox[origin=c]{90}{Source}}  
%                           & RCH  &   \textbf{0.9447}*    &    0.9109*   &   0.9498   &  \\
%                           & GCH  &   0.9367*    &   \textbf{0.8697}    &      0.9337*   &    \\

% \end{tabular}
%  \begin{center}
%       \small {* 10-fold cross validation}
%   \end{center}
% \end{table}


